Swarical: An Integrated Hierarchical Approach to Localizing Flying Light Specks

Swarical, a Swarm-based hierarchical localization technique, enables miniature drones, known as Flying Light Specks (FLSs), to accurately and efficiently localize and illuminate complex 2D and 3D shapes. Its accuracy depends on the physical hardware (sensors) of FLSs, which are used to track neighboring FLSs in order to localize themselves. It uses the hardware specification to convert mesh files into point clouds that enable a swarm of FLSs to localize at the highest accuracy afforded by their hardware. Swarical considers a heterogeneous mix of FLSs with different orientations for their tracking sensors, ensuring a line of sight between a localizing FLS and its anchor FLS. We present an implementation using Raspberry cameras and ArUco markers. A comparison of Swarical with a state of the art decentralized localization technique shows that it is as accurate and more than 2x faster.

==> RaspberryModel.tex <==
\begin{figure}
    \centering
    \includegraphics[width=\columnwidth]{figs/percentageDistErrWide2cmMerkerEX.jpg}
    \caption{Percentage error in distance measurement at millimeter granularity, 569-123 millimeters, wide lens, 20 mm paper-printed marker size.}
    \label{fig:dist_error_sweet}
\end{figure}


\begin{figure}
    \centering
    \includegraphics[width=\columnwidth]{figs/orientationErrWide2cmMerkerEX.jpg}
    \caption{Orientation error in degrees at millimeter granularity, 59-123 millimeters, wide lens, 20 mm paper-printed marker size.}
    \label{fig:orientation_error_sweet}
\end{figure}

The Raspberry camera provides millimeter accuracy in the range of 6 to 8 cm.
Figure~\ref{fig:dist_error_sweet} shows the percentage error in distance for this range at millimeter granularity.
The maximum error is 1.2\%. 
The orange line shows the following quadratic function that models the gathered data: 
\[f_{dist}(x)=-0.00331703179 x^2 + 0.480304854 x - 16.6922920\].

The observed error in orientation is less than 1.2 degrees, see Figure~\ref{fig:orientation_error_sweet}.
%The highest error is observed in the roll.  
%Measuring Yaw is most accurate in our experimental setup.
The difference in error observed with the roll, pitch, and yaw is experimental noise attributed to the manual setup of the marker and camera.
For the range of 6 to 8 cm, the following quadratic functions model the error as a function of the distance:
\[f_{roll}(x)=-0.000588533106 x^2 + 0.0746982216 x - 1.15565179\]
\[f_{pitch}(x)=0.000218285194 x^2 - 0.0373837587 x + 2.26655293\]
\[f_{yaw}(x)=0.00000553090683 x^2 + 0.00486011610 x - 0.167660009\]

Figures \ref{fig:dist_error_sweet} and \ref{fig:orientation_error_sweet} are based on the wide lens camera with 16 frames per second rate and 720p resolution.

==> camera.tex <==
Localization of two FLSs relative to each other is sensitive to the errors in the relative position and orientation measurements. We evaluated relative position and orientation estimation using ArUco markers and Raspberry cameras to provide insight into the accuracy of this technique.
The ideal camera should be small, light-weight, and ready for use with a drone. Table~\ref{tab:cameras} lists the cameras we used and their specifications. We utilized Raspberry Camera Module 3 NoIR (\$25) and Raspberry Camera Module 3 NoIR Wide (\$35). The wide camera has a focus range of 5cm-$\infty$ and a diagonal field of view of 120 degrees compared to the 8cm-$\infty$ focus range and 75 diagonal field of view of the regular camera. Both cameras have 4608 x 2592 pixels image sensors and an automatic focus. Image sensors have different sensor modes in which they can operate. Different modes produce different image resolutions and fields of view. We report the frame rate for the experiments we conducted.
To display ArUco markers we considered a 1.3-inch LCD and printed markers. 


Objective: Insight into the accuracy of this technique.

Motivation:  Relative localization is sensitive to the error in distance and measured angles.  Both are equally important.

{\bf Todo: } 
\begin{enumerate}
    \item Include the table from Slide 48.  {\bf Provide a table that highlights these parameters for the two cameras considered in this study.}
    \item List of cameras comparable to those that were evaluated in this study?
\end{enumerate}

The ideal camera should be small, light weight, and ready for use with a drone.  We consider two such cameras in this study.  

Hardware and Software Setup:  
Hardware: 
\begin{enumerate}
\item Camera specs:  We analyzed a camera with a wide angle (\$35) lens and compared it with a camera that has regular lens (\$25).  Different min/max distances with the different cameras.  Other important specifications:
FoV, resolution, focus range, Macro, Frame rate.
FoV is defined as XXX~\cite{}.
Resolution is defined as the number of pixels on the image sensor.
Focus range is the min/max which depends on the lens. 
Macro lens produces an image that is the size of an object. 
It has a 1 to 1 production ratio.  
Frame rate of the camera:

\item {\bf Is it known that the lens of the camera makes a difference when it comes to min/max distance?}

\item Marker size using paper and as displayed on LCD:
LCD is generally more accurate than paper in measuring both distance and angle. 
{\bf To do: Why is it better?}

\item Raspberry PI 5 with 4 Gigabytes of RAM.  Software:
OpenCV that includes off-the-shelf software to process fiducial markers.

\item Infrared light.  {\bf Todo: Size and price of LED? 
 5m, \$0.27, 940 nm wavelength.}
\end{enumerate}

Results:
\begin{itemize}
\item 1. Observed error with minimum distance of 5 cm < 1\%.
\item 2. Accuracy is independent of the frame rate:  What is the percentage error in distance/angle as a function of the frame rate? 
\item 2. Trend 1:  Item 1 depends on the marker size.  With a fixed distance, a larger marker reduce the amount of error dramatically.  It is 0.01\%.
\item 3. What is the maximum distance with the marker used to measure distance of 5 cm? 44 cm with a different camera (the minimum distance with this camera is 10 cm).  TO DO: MEASURE MAX DISTANCE WITH CAMERA THAT HAS MIN DISTANCE OF 5 CM.  Why does the camera matter for the distance?  
\item 4. Angle error is within 1 to 2 degrees.  {\bf Todo: 
 Gather results for the regular lens to include in the paper.}
 \item 5. {\bf Todo:  Measure error in distance and angle with Infrared.}
\end{itemize}

Rationalization about reducing the size of the camera which in turn reduces the size of the marker. 

FLSs must operate in both dark rooms and regularly lit room.  Infrared was used to light up the environment without being visible to the human eye.  Idea:  Come up with a marker invisible with regular light but visible with infrared light.  {\bf Todo:  The idea remains to be tested.  Given the lack of time, we may push this idea to the future work section.}


==> evalOLD.tex <==
%Describe the implementation using the CloudLab and Amazon AWS.Describe the number of cores used to conduct the experiments.

%Obtained results show:
%\begin{itemize}
%    \item Small swarm sizes ($G \leq$10) result in illuminations with a large amount of error.
%    \item ISR is superior to HC and RSF.
%\end{itemize}

%How is the ArUco marker mounted on an FLS? 

%How many kinds of ArUco markers are there? 
  
%How is the error in orientation as a function of distance is modeled? 


\subsection{Planner}\label{sec:evalplanner}
%Can we show the different versions of the Skateboard with different sampling techniques?

We use the range of the Raspberry camera at [6,8] cm as it provides the highest accuracy. 
With this range, the planner computes a point cloud of 1855 FLSs for the skateboard. 
The mix of FLSs with a camera mounted on their top, side, and bottom is 152, 1585, and 118, respectively.
The percentage of each variant is 8.2\%, 85.4\%, and 6.4\%, respectively.
This mix ensures a localizing FLS has line of sight with the ArUco marker of its anchor FLS. 
With all the shapes, the percentage of FLSs with a camera mounted on their side is significantly higher than the others. 

\begin{figure}
    \centering
    \includegraphics[width=\columnwidth]{figs/planner/SkateboardSwarmSize_G50_2.jpg}
    \caption{Distribution of swarm size, Skateboard, $G$=50.}
    \label{fig:planner-swarm-size}
\end{figure}
Figure~\ref{fig:planner-swarm-size} shows the distribution of swarm size with the Skateboard with $G$=50.
Swarical uses k-Means to construct swarms. 
This clustering technique minimizes the eucledian distance between the FLSs that constitute a swarm.
However, it does not ensure swarms of the size. 
As shown, the size of a swarm varies from 10 to 90.
The same is true with the other shapes.
The topology of a shape dictates the swarm sizes constructed by k-means.

 

Figure~\ref{fig:planner-dist} shows the distribution of distance between localizing and anchor FLSs within the swarms (FLS-trees) and across swarms (swarm-tree).
This is for the skateboard with different group sizes, $G$.
In these experiments, the planner was configured to limit the distance between a localizing and an anchor FLS to [6-8] cm.
After constructing the swarm-tree and FLS-trees for each value of $G$,
It injected a total of 160, 132, 40, 23 and 18 FLSs for $G$=5, 10, 50, 150, and 200, respectively. 
Hence, the median is between 6 and 7 cm for all $G$ values.
There is no localizing-anchor pair with a distance smaller than 6 cm.
The variation in distance is greater for the swarm-tree with smaller group sizes, $G$=5 and 10. 
This is because there is a larger number of swarms.
The inverse is observed with larger group sizes, $G$=150 and 200, because there are fewer swarms.


\begin{figure}
    \centering
    \includegraphics[width=\columnwidth]{figs/planner/SkateboardDistanceBox_2.jpg}
    \caption{Distribution of distance between localizing and anchor FLSs within a swarm (FLS-tree) and across swarms (Swarm-tree), Skateboard.}
    \label{fig:planner-dist}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[width=\columnwidth]{figs/planner/SkateboardBranchingFactorBox_2.jpg}
    \caption{Distribution of the number of localizing FLSs (swarms) per anchor FLS, Skateboard.}
    \label{fig:planner-branch}
\end{figure}


Figure~\ref{fig:planner-branch} shows the distribution of the branching factor for the swarm-tree and the FLS-trees.
This is the number of FLSs (swarms) that localize relative to one anchor FLS (swarm).
The median is one.
However, the outliers may be as high as 3 or 4.
The minimum is zero.
These correspond to FLSs (swarms) that are the leaves of an FLS-tree (swarm-tree). 


\subsection{Localization}\label{sec:evallocalize}
We use Hausdorff Distance (HD)~\cite{Huttenlocher93} and Chamfer Distance (CD)~\cite{chamfer2017} to  compare the FLS coordinates obtained using a localization technique, i.e., the estimated truth E, with the FLS coordinates provided by the Planner, i.e., the ground truth $P$.
HD quantifies the maximum error in distance between $E$ and $P$ after applying a translation.
CD quantifies the average error between $E$ and $P$.
Both techniques require a 
translation process because Swarical is a relative localization technique.
Our implementation of the translation process computes the center of $E$ and $P$.  
It aligns their centers prior to measuring the maximum/average error. 
A lower value is better with zero reflecting a perfect match between $E$ and $P$.

In general, HD is more strict that CF because it uses the maximum error.
Both are useful in understanding the tradeoffs associated with the alternative techniques. 

\begin{figure}
    \centering
    \begin{subfigure}{\columnwidth}
        \includegraphics[width=\textwidth]{figs/results/SkateboardVariantComparison_HD_G50.jpg}
        \caption{Hausdorff Distance.}
        \label{fig:cmp_hd}
    \end{subfigure}

    \begin{subfigure}{\columnwidth}
        \includegraphics[width=\textwidth]{figs/results/SkateboardVariantComparison_CD_G50.jpg}
        \caption{Chamfer Distance.}
        \label{fig:cmp_cd}
    \end{subfigure}

    \caption{Comparison of different techniques with the Skateboard and $G=50$.}
    \label{fig:sk_var_comp}
\end{figure}

% with error model
\begin{figure}
    \centering
    \begin{subfigure}{\columnwidth}
        \includegraphics[width=\textwidth]{figs/results/SkateboardVariantComparison_HD_G50_werr.jpg}
        \caption{Hausdorff Distance.}
        \label{fig:cmp_hd}
    \end{subfigure}

    \begin{subfigure}{\columnwidth}
        \includegraphics[width=\textwidth]{figs/results/SkateboardVariantComparison_CD_G50_werr.jpg}
        \caption{Chamfer Distance.}
        \label{fig:cmp_cd}
    \end{subfigure}

    \caption{Comparison of different techniques with the Skateboard and $G=50$.}
    \label{fig:sk_var_comp_err}
\end{figure}

Figure~\ref{fig:sk_var_comp} compares HC, ISR and RSF with one another.
The x-axis is the elapsed time from when the dispatcher deploys the first FLS.
Once an FLS arrives at its assigned coordinate, it starts to localize.
We assume a 5° dead reckoning error.  
The y-axis shows the HD and the CD in Figure~\ref{fig:cmp_hd} and~\ref{fig:cmp_cd}, respectively.
Both figures are for the Skateboard with $G$=50.
Similar trends are observed with the other shapes and values of $G$.

Figure~\ref{fig:sk_var_comp} shows ISR is superior to HC and RSF.
It enhances both HD and CD, providing illuminations that resemble those computed by the Planner more accurately.

RSF is inferior and slow in reducing HD and CD for two reasons.
First, its intra-group localization is slower.
RSF uses the hierarchy of an FLS-tree to guide the localization of FLSs in a swarm.
With HC and ISR, the FLSs in a swarm localize independently. 
Second, RSF initiates localization with the root of the swarm-tree and must walk down all the swarms and their FLS-trees.
Both design decisions slow down the localization process.
%The leaf swarms of the swarm-tree and their parents localize more than the root swarm. This is because the likelihood of their anchor FLS moving is higher every time a swarm close to the top of the tree localizes. 

RSF's HD improves suddenly\footnote{In less than one Second.} at the 48$^{th}$ Second of Figure~\ref{fig:cmp_hd}.
This occurs once a leaf swarm of the swarm-tree performs an inter-swarm localization relative to its parent swarm.
Its entire swarm moves into a more accurate pose relative to all the swarms, resulting in a significant improvement in accuracy, i.e., drop in HD and CD.

{\bf Why does HC's HD starts to level off and increase?}
One FLS stops localizing.  
This FLS is the primary of a swarm.
The swarm is the grandchild of the root swarm. 
This swarm has 60 FLSs.
What is the distance between the primary and its anchor?  

In all these experiments, RSF causes the FLSs to travel a longer total distance when compared with ISR and HC.
ISR reduces this metric slightly lower than HC. 
This slight improvement is consistent throughout our experiments. 

\begin{figure}
    \centering
    \begin{subfigure}{\columnwidth}
        \includegraphics[width=\textwidth]{figs/results/SkateboardGroupSizeComparison_HD_ISR.jpg}
        \caption{Hausdorff Distance.}
        \label{fig:hd}
    \end{subfigure}

    \begin{subfigure}{\columnwidth}
        \includegraphics[width=\textwidth]{figs/results/SkateboardGroupSizeComparison_CD_ISR.jpg}
        \caption{Chamfer Distance.}
        \label{fig:cd}
    \end{subfigure}

    \caption{Comparison of different swarm sizes ($G$) with the Skateboard and the ISR technique. Lower is better.}
    \label{fig:ISR_var_comp}
\end{figure}

% with error model
\begin{figure}
    \centering
    \begin{subfigure}{\columnwidth}
        \includegraphics[width=\textwidth]{figs/results/SkateboardGroupSizeComparison_HD_ISR_werr.jpg}
        \caption{Hausdorff Distance.}
        \label{fig:hd}
    \end{subfigure}

    \begin{subfigure}{\columnwidth}
        \includegraphics[width=\textwidth]{figs/results/SkateboardGroupSizeComparison_CD_ISR_werr.jpg}
        \caption{Chamfer Distance.}
        \label{fig:cd}
    \end{subfigure}

    \caption{Comparison of different swarm sizes ($G$) with the Skateboard and the ISR technique. Lower is better.}
    \label{fig:ISR_var_comp}
\end{figure}

Figure~\ref{fig:ISR_var_comp} shows the HD and CD of the Skateboard with ISR and different swarm sizes ($G$).
Small swarm sizes ($G\leq$10) result in a higher HD and CD, i.e., a larger difference between the FLS clouds illuminated by ISR and the FLS cloud computed by the Swarical's planner.
This is because they result in a larger number of swarms that is unbalanced and deep, 43 with $G$=5 and 38 with\footnote{Depth decreases to 12 with $G$=50.} $G$=10.
The swarms close to the leaves of the swarm-tree require a longer time to localize because their anchor in a parent swarm has a higher probability of changing its location.
This change is due to both intra-swarm and inter-swarm localization.
An inter-swarm localization of a primary moves the entire swarm including those FLSs that serve as anchors for other swarms.
These result in a high Hausdorff and Chamfer distances.

With $G$=150, the HD levels off because XXX.
However, its CD is competitive.  Why?
Leaf FLS in a leaf swarm.
It stops localizing.

\subsection{A Comparison with SwarMer}\label{sec:cmpSwarMer}
SwarMer~\cite{alimohammadzadeh2023swarmer} is a decentralized localization framework for FLSs.
Individual FLSs localize relative to one another to form swarms. 
An FLS of one swarm localizes relative to an anchor FLS of another swarm to merge with it, forming a larger swarm.
This process repeats, causing swarms to merge until there is one swarm.
Subsequently, SwarMer thaws the final swarm into individual FLSs and repeats the process again.

Both SwarMer and Swarical are continuous techniques that use the concept of localizing and anchor FLSs.
SwarMer constructs its swarms in an online manner.
Swarical is different because it constructs its swarms in an offline manner.
SwarMer's swarms are seeded with 1 FLS that merge to construct larger swarms, ultimately growing into one swarm that includes all FLSs.
%At this point, SwarMer thraws the swarm and starts over with small swarms consisting of 1 FLS. 
Swarical's swarms are static.
Swarical is an integrated approach that considers the range of sensors mounted on an FLS to track another FLS.
This is reflected in its hierarchical swarm-tree and $nG$ FLS-trees.
These concepts are absent from SwarMer.
%Similarly, SwarMer's concept of merging small swarms into one large swarm that includes all FLSs is absent from Swarical.

Figure~\ref{fig:swarmer_Swarical} shows the HD with SwarMer and Swarical for the Skateboard.
Swarical is configured with
group size is 50 ($G$=50) and the ISR technique.
SwarMer does not consider the error associated with the range of an FLS's tracking device.
Hence, we assumes the tracking device is 100\% accurate in measuring the pose of an FLS.
These results show Swarcial localizes the FLSs more than 2x faster than SwarMer. 
A similar observation is made with CD.

Swarical is faster than SwarMer for two reasons.
First, FLSs exchange fewer messages.
More specifically, 
SwarMer requires a challenge phase for a localizing FLS to identify its anchor FLS. 
This step is absent from Swarmical; its Planner computes the localizing and anchor FLSs in an offline manner.
Second, FLSs move a shorter distance with Swarical when compared with SwarMer.
In the experiments of Figures~\ref{fig:swarmer_Swarical}, on the average 8\% less.
The minimum distance moved by FLSs with Swarmical is 12\% shorter than SwarMer.




%Swarmer:  min:57.8, max:307.7, avg:162 cm

%Swarical: min:51.6, max:275.9, avg:149.5 cm

\begin{figure}
    \centering
    \includegraphics[width=\columnwidth]{figs/results/SkateboardSwarMerISRComparison_HD.jpg}
    \caption{Comparison of Swarical with SwarMer for the Skateboard.}
    \label{fig:swarmer_Swarical}
\end{figure}

==> fig1.tex <==
 \begin{figure}[htbp]
    \centering
    \captionsetup[subfigure]{justification=centering}
    \begin{subfigure}{0.24\columnwidth}
        \centering
        \includegraphics[width=\textwidth]{figs/racecar_3720_gtl_691.png}
        \caption{Racecar, \\3720.}
    \end{subfigure}
        \begin{subfigure}{0.24\columnwidth}
        \centering
        \includegraphics[width=0.9\textwidth]{figs/skateboard_1372_gtl_635.png}
        \caption{Skateboard, \\1372.}
    \end{subfigure}
    \begin{subfigure}{0.24\columnwidth}
        \centering
        \includegraphics[width=0.9\textwidth]{figs/kangaroo_972_gtl_636.png}
        \caption{Kangaroo, \\972.}
    \end{subfigure}
    \begin{subfigure}{0.24\columnwidth}
        \centering
        \includegraphics[width=0.3\textwidth]{figs/chess_408_gtl_234.png}
        \caption{Chess, \\408.}
    \end{subfigure}


    \caption{Four point clouds and their number of FLSs.} 
    \label{fig:shapes} 
\end{figure}

==> models.tex <==
We introduce three distinct error models designed to simulate the uncertainty inherent in distance. 
%measurement using signal strength.

Model 1, Fixed Percentage Error Model: This model introduces a consistent error margin in the distance estimation. Under this model, every measurement is subject to a fixed percentage deviation x from the ground truth. This deviation is consistent across all measurements, regardless of the actual distance or signal strength. For instance, if the fixed error is set at $\pm 5\%$, and the ground truth distance is 100 cm, the measured distance would fluctuate between 95 and 105 cm. This model is beneficial for understanding the impact of a constant error rate across different distances.

Model 2, Probabilistic Absolute Error Model: This model incorporates a probabilistic element in the error estimation. It assumes that the measurement is 100\% accurate with a certain probability
p (i.e., no error). Conversely, with a probability of 1-p, the measurement deviates from the ground truth by a fixed percentage x. For example, if 
p is 0.8 (or 80\%), there is an 80\% chance that the measurement is completely accurate and a 20\% chance that it is off by $e \in [-x, +x]$ from the ground truth. This model reflects scenarios where measurements are generally reliable but are occasionally subject to significant errors.

Model 3, Probabilistic Variable Error Model: Similar to the second model, this model also assigns a probability p to the likelihood of a measurement being accurate. However, unlike the previous model, the error in this model is not a fixed percentage but varies unpredictably. With a probability of 1-p, the measurement error is an unknown percentage, introducing a higher level of uncertainty. This model is particularly useful in situations where the error in the measurement is not only probable but also variable and unpredictable.

==> swarmer.tex <==
SwarMer is designed to enable a swarm of devices to render complex 2D and 3D shapes.
An example device is a Flying Light Speck, FLS, a miniature sized drone configured with light sources to generate different colors and textures with adjustable brightness~\cite{shahram2021,shahram2022}.
An FLS is unable to render a shape by itself.
SwarMer uses the inter-FLS relationship effect of its organizational framework to compensate for the simplicity of each individual FLS, enabling a swarm of cooperating FLSs to render complex shapes.

SwarMer is a relative localization technique.
Given a 2D or 3D point cloud, it approximates the position of the FLSs by forcing the neighboring FLSs to match the relative distance and angle~\cite{deter2022} of their assigned points.  Even though the location of each FLS is not exactly the same as that specified by the point cloud, SwarMer’s relative positioning of FLSs produces shapes true to a point cloud.

SwarMer is a continuous technique.  It requires an FLS to localize relative to an anchor FLS, merging their swarms into one.  If each of the localizing FLS and anchor FLS is associated with a swarm then the two swarms merge into one.  When there is a single swarm, SwarMer thaws the swarm to form individual devices.  It repeats the process of an FLS localizing relative to an anchor FLS, forming swarms.  This repetition enables SwarMer to localize FLSs with a high accuracy.  We quantify the error in the estimated truth (location of FLSs using SwarMer) with the ground truth (the point cloud) using the Hausdorff Distance, HD~\cite{Huttenlocher93}.
In our experiments, SwarMer reduces HD aggressively to below 0.01 as it constructs and thaws swarms in less than a minute.
With HD $\leq$ 0.01, the movement of localizing FLSs is not noticable because each FLS moves by a very small distance.

\begin{figure}
\centering
\includegraphics[width=\columnwidth]{figs/vectors.png}
\caption{$\vec{V}$ shows the dead-reckoning movement and $\vec{d}$ shows the distance between FLSs.}
\label{fig:vectors}
\end{figure}

SwarMer is a framework that requires a relative localization technique for use by an FLSs.
A technique may mount sensors on the FLSs and use their Signal Strength (SS) to detect both the angle and the distance between a pair of FLSs.
See Figure~\ref{fig:vectors}.
In this figure, a localizing FLS (in gray) uses SS to measure its distance to an anchor FLS, $\vec{d}$.  It knows what this distance should be in the ground truth (coordinates of a point cloud), $\vec{D}$.
Using these two pieces of information along with the angles $\alpha$ and $\theta$, it computes a Vector $\vec{V}$ and moves along this vector to a new location.

This paper focuses on Vectors $\vec{d}$ and $\vec{V}$ and the error in their distances.
These distances are termed Measure Distance (MD) and Travelled Distance (TD).
Vector $\vec{d}$ is the Measured Distance (MD) between the current position of a localizing FLS and the anchor FLS.
The Distance Travelled (DT) by a drone is defined by Vector $\vec{V}$.
Both distances are susceptible to error.
While one may use a sampling technique with MD, the FLS movement along vector $\vec{V}$ is final and DT not be sampled.
We wondered if the continuous property of SwarMer enables it to overcome the different forms of error in MD and DT.  And, if affirmative, what percentage error can be tolerated.
This information is useful in two ways.  First, it guides the selection of a relative localization technique among multiple choices.  Second, it motivates extensions of SwarMer to tolerate error produced by a relative localization technique.


\begin{table}[ht]
\centering
\renewcommand{\arraystretch}{1.5} % Increase the row height by 50%
\caption{This table summarizes our findings.  }
\begin{tabular}{|c|c|c|c|}
\hline
\multirow{2}{*}{\textbf{Distance}} & \multicolumn{3}{c|}{\textbf{Error Models}} \\
\cline{2-4}
 & \textbf{Model 1} & \textbf{Model 2} & \textbf{Model 3} \\
\hline
\textbf{Distance Travelled (DT), $\vec{V}$} & \textcolor{Green}{\checkmark} & \textcolor{Green}{\checkmark} & \textcolor{Green}{\checkmark} \\
\hline
\textbf{Measured Distance (MD), $\vec{d}$} & \textcolor{Red}{\texttimes} & \textcolor{Green}{\checkmark} & \textcolor{Green}{\checkmark} \\
\hline
\end{tabular}
\label{tab:grid}
\end{table}



The {\bf contributions} of this paper are:
\begin{itemize}
\item A sensitivity analysis of SwarMer to different forms of error and percentage errors in distance quantified by a relative localization technique.
\item Obtained results show..., see Table~\ref{tab:grid}.
\end{itemize}


